Joint Modeling of Feature, Correspondence, and a Compressed Memory for Video Object Segmentation

Current prevailing Video Object Segmentation methods follow the pipeline of extraction-then-matching, which first extracts features on current and reference frames independently, and then performs dense matching between them. This decoupled pipeline limits information propagation between frames to high-level features, hindering fine-grained details for matching. Furthermore, the pixel-wise matching lacks holistic target understanding, making it prone to disturbance by similar distractors. To address these issues, we propose a unified VOS framework, coined as JointFormer, for jointly modeling feature extraction, correspondence matching, and a compressed memory. The core Joint Modeling Block leverages attention to simultaneously extract and propagate the target information from the reference frame to the current frame and a compressed memory token. This joint scheme enables extensive multi-layer propagation beyond high-level feature space and facilitates robust instance-distinctive feature learning. To incorporate the long-term and holistic target information, we introduce a compressed memory token with a customized online updating mechanism, which aggregates target features and facilitates temporal information propagation in a frame-wise manner, enhancing global modeling consistency. Our JointFormer achieves a new state-of-the-art performance on the DAVIS 2017 val/test-dev (89.7\% and 87.6\%) benchmarks and the YouTube-VOS 2018/2019 val (87.0\% and 87.0\%) benchmarks, outperforming the existing works. To demonstrate the generalizability of our model, it is further evaluated on four new benchmarks with various difficulties, including MOSE for complex scenes, VISOR for egocentric videos, VOST for complex transformations, and LVOS for long-term videos.

==> Letter.tex <==
Dear Editor and Reviewers of T-PAMI,

We are submitting a manuscript entitled “JointFormer: A Compact Framework with Joint Modeling for Video Object Segmentation” for your consideration for publication in the journal of T-PAMI. This journal version has been written from scratch and all the authors listed have approved the manuscript that is enclosed.

This work aims to design a compact and concise framework with joint modeling and we present four major contributions:

1. We propose a unified network, coined as JointFomer, to jointly model feature, correspondence, and a compressed memory. The compact and concise framework enables extensive information propagation and discriminative learning.
2. We develop a customized online updating mechanism for the compressed memory, which helps to prompt the information flow along the temporal dimension and thus providing a long-term adaptive feature and improving global modeling capability.
3. Comprehensive experiments show that our JointFomer achieves state-of-the-art performance with 89.7% and 87.6% on DAVIS 2017 validation and test-dev split, 87.0% and 87.0% on YouTube-VOS 2018 & 2019 validation split. In addition, we test our JointFormer on four new benchmarks with various difficulties, including MOSE, VOST, VISOR, and LVOS, and compare it to three current best models. The results show that we achieve the best performance on all four benchmarks, indicating that our model is able to overcome various challenges.

Sincerely yours,
Jiaming Zhang, YuTao Cui, Gangshan Wu, and Limin Wang

==> tables_ablations/ConvMAE_FPS.tex <==
\begin{tabular}{l|ccc}
\toprule[1.5pt]
Method & $Y_{18}^{val}$ & Fps & Mem \\
\midrule[1pt]
AOT-L$^{\diamond}$    & 78.8 & 4.9 & 17847            \\
DeAOT-L$^{\diamond}$  & 83.5 & 7.6 & 6144            \\
XMem$^{\diamond}$  & 85.3 & 25.5 & 1877            \\
\midrule[1pt]
Ours - 1         & 85.8 & 6.7 & 4404           \\
Ours - 2         & 86.0 & 3.6 & 5030           \\
\textbf{Ours - 3}         & 86.0 & 3.0 & 5785           \\
\bottomrule[1.5pt]
\end{tabular}

